e-Profits: A Business-Aligned Evaluation Metric for Profit-Sensitive Customer Churn Prediction

Retention campaigns in customer relationship management often rely on churn prediction models evaluated using traditional metrics such as AUC and F1-score. However, these metrics fail to reflect financial outcomes and may mislead strategic decisions. We introduce e-Profits, a novel business-aligned evaluation metric that quantifies model performance based on customer lifetime value, retention probability, and intervention costs. Unlike existing profit-based metrics such as Expected Maximum Profit, which assume fixed population-level parameters, e-Profits uses Kaplan-Meier survival analysis to estimate tenure-conditioned (customer-level) one-period retention probabilities and supports granular, per-customer profit evaluation. We benchmark six classifiers across two telecom datasets (IBM Telco and Maven Telecom) and demonstrate that e-Profits reshapes model rankings compared to traditional metrics, revealing financial advantages in models previously overlooked by AUC or F1-score. The metric also enables segment-level insight into which models maximise return on investment for high-value customers. e-Profits provides a transparent, customer-level evaluation framework that bridges predictive modelling and profit-driven decision-making in operational churn management. All source code is available at: https://github.com/Awaismanzoor/eprofits.

==> Bib.tex <==
\begin{thebibliography}{10}
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\expandafter\ifx\csname href\endcsname\relax
  \def\href#1#2{#2} \def\path#1{#1}\fi

\bibitem{van2004customer}
D.~Van~den Poel, B.~Lariviere, Customer attrition analysis for financial services using proportional hazard models, European journal of operational research 157~(1) (2004) 196--217.

\bibitem{zhou2023early}
Y.~Zhou, W.~Chen, X.~Sun, D.~Yang, Early warning of telecom enterprise customer churn based on ensemble learning, Plos one 18~(10) (2023) e0292466.

\bibitem{ganesh2000understanding}
J.~Ganesh, M.~J. Arnold, K.~E. Reynolds, Understanding the customer base of service providers: an examination of the differences between switchers and stayers, Journal of marketing 64~(3) (2000) 65--87.

\bibitem{sun2021case}
Y.~Sun, Case based models of the relationship between consumer resistance to innovation and customer churn, Journal of Retailing and Consumer Services 61 (2021) 102530.

\bibitem{loureiro2025improving}
A.~Loureiro, V.~Migueis, A.~Costa, M.~Ferreira, Improving customer retention in taxi industry using travel data analytics: A churn prediction study, Journal of Retailing and Consumer Services 85 (2025) 104288.

\bibitem{kotan2025novel}
M.~Kotan, {\"O}.~Faruk~Seymen, L.~{\c{C}}all{\i}, S.~Kas{\i}m, B.~{\c{C}}arkl{\i}~Yavuz, T.~{\"O}ver~{\"O}z{\c{c}}elik, A novel methodological approach to saas churn prediction using whale optimization algorithm, PloS one 20~(5) (2025) e0319998.

\bibitem{peng2023research}
K.~Peng, Y.~Peng, W.~Li, Research on customer churn prediction and model interpretability analysis, Plos one 18~(12) (2023) e0289724.

\bibitem{faraji2024customer}
K.~Faraji~Googerdchi, S.~Asadi, S.~M. Jafari, Customer churn modeling in telecommunication using a novel multi-objective evolutionary clustering-based ensemble learning, Plos one 19~(6) (2024) e0303881.

\bibitem{hand2009measuring}
D.~J. Hand, Measuring classifier performance: a coherent alternative to the area under the roc curve, Machine learning 77~(1) (2009) 103--123.

\bibitem{elkan2001foundations}
C.~Elkan, The foundations of cost-sensitive learning, in: International joint conference on artificial intelligence, Vol.~17, Lawrence Erlbaum Associates Ltd, 2001, pp. 973--978.

\bibitem{bahnsen2015novel}
A.~C. Bahnsen, D.~Aouada, B.~Ottersten, A novel cost-sensitive framework for customer churn predictive modeling, Decision Analytics 2 (2015) 1--15.

\bibitem{thakkar2022clairvoyant}
H.~K. Thakkar, A.~Desai, S.~Ghosh, P.~Singh, G.~Sharma, Clairvoyant: Adaboost with cost-enabled cost-sensitive classifier for customer churn prediction, Computational intelligence and neuroscience 2022~(1) (2022) 9028580.

\bibitem{rahman2025profit}
S.~Rahman, B.~Janssens, M.~Bogaert, Profit-driven pre-processing in b2b customer churn modeling using fairness techniques, Journal of Business Research 189 (2025) 115159.

\bibitem{lemmens2020managing}
A.~Lemmens, S.~Gupta, Managing churn to maximize profits, Marketing Science 39~(5) (2020) 956--973.

\bibitem{verbeke2012new}
W.~Verbeke, K.~Dejaeger, D.~Martens, J.~Hur, B.~Baesens, New insights into churn prediction in the telecommunication sector: A profit driven data mining approach, European journal of operational research 218~(1) (2012) 211--229.

\bibitem{verbraken2012novel}
T.~Verbraken, W.~Verbeke, B.~Baesens, A novel profit maximizing metric for measuring classification performance of customer churn prediction models, IEEE transactions on knowledge and data engineering 25~(5) (2012) 961--973.

\bibitem{bhattacharyya2021investigation}
J.~Bhattacharyya, M.~K. Dash, Investigation of customer churn insights and intelligence from social media: A netnographic research, Online Information Review 45~(1) (2021) 174--206.

\bibitem{mena2024exploiting}
G.~Mena, K.~Coussement, K.~W. De~Bock, A.~De~Caigny, S.~Lessmann, Exploiting time-varying rfm measures for customer churn prediction with deep neural networks, Annals of Operations Research 339~(1) (2024) 765--787.

\bibitem{ly2022churn}
T.~V. Ly, D.~V.~T. Son, Churn prediction in telecommunication industry using kernel support vector machines, Plos one 17~(5) (2022) e0267935.

\bibitem{tavassoli2022hybrid}
S.~Tavassoli, H.~Koosha, Hybrid ensemble learning approaches to customer churn prediction, Kybernetes 51~(3) (2022) 1062--1088.

\bibitem{sana2022novel}
J.~K. Sana, M.~Z. Abedin, M.~S. Rahman, M.~S. Rahman, A novel customer churn prediction model for the telecommunication industry using data transformation methods and feature selection, Plos one 17~(12) (2022) e0278095.

\bibitem{stripling2018profit}
E.~Stripling, S.~vanden Broucke, K.~Antonio, B.~Baesens, M.~Snoeck, Profit maximizing logistic model for customer churn prediction using genetic algorithms, Swarm and Evolutionary Computation 40 (2018) 116--130.

\bibitem{oskarsdottir2018profit}
M.~{\'O}skarsd{\'o}ttir, B.~Baesens, J.~Vanthienen, Profit-based model selection for customer retention using individual customer lifetime values, Big data 6~(1) (2018) 53--65.

\bibitem{hoppner2020profit}
S.~H{\"o}ppner, E.~Stripling, B.~Baesens, S.~vanden Broucke, T.~Verdonck, Profit driven decision trees for churn prediction, European journal of operational research 284~(3) (2020) 920--933.

\bibitem{perianez2016churn}
{\'A}.~Peri{\'a}{\~n}ez, A.~Saas, A.~Guitart, C.~Magne, Churn prediction in mobile social games: Towards a complete assessment using survival ensembles, in: 2016 IEEE International Conference on Data Science and Advanced Analytics (DSAA), 2016, pp. 564--573.

\bibitem{xu2022lads}
F.~Xu, H.~Zhang, J.~Zheng, T.~Ting~Zhao, X.~Dong~Wang, Z.~Yong~Zeng, \href{https://doi.org/10.1145/3529836.3529853}{Lads: Deep survival analysis for churn prediction analysis in the contract user domain}, in: Proceedings of the 2022 14th International Conference on Machine Learning and Computing, ICMLC '22, Association for Computing Machinery, New York, NY, USA, 2022, p. 237–244.
\newblock \href {https://doi.org/10.1145/3529836.3529853} {\path{doi:10.1145/3529836.3529853}}.
\newline\urlprefix\url{https://doi.org/10.1145/3529836.3529853}

\bibitem{garcia2017intelligent}
D.~L. Garc{\'\i}a, {\`A}.~Nebot, A.~Vellido, Intelligent data analysis approaches to churn as a business problem: a survey, Knowledge and Information Systems 51~(3) (2017) 719--774.

\bibitem{manzoor2024review}
A.~Manzoor, M.~Atif~Qureshi, E.~Kidney, L.~Longo, A review on machine learning methods for customer churn prediction and recommendations for business practitioners, IEEE Access 12 (2024) 70434--70463.

\bibitem{rahman2024ibm}
H.~Rahman, R.~P. Afrianto, F.~Mohammad, D.~A. Tajriyaani, R.~A.~N. Azhar, Ibm telco customer churn prediction with survival analysis, in: Proceedings of the International Conference on Advanced Technology and Multidiscipline (ICATAM 2024)., Vol. 245, Springer Nature, 2024, p. 386.

\bibitem{stevens2020comparing}
N.~T. Stevens, L.~Lu, Comparing kaplan-meier curves with the probability of agreement, Statistics in Medicine 39~(30) (2020) 4621--4635.

\bibitem{liu2023concrete}
G.~Liu, B.~Sun, Concrete compressive strength prediction using an explainable boosting machine model, Case Studies in Construction Materials 18 (2023) e01845.

\bibitem{bentejac2021comparative}
C.~Bent{\'e}jac, A.~Cs{\"o}rg{\H{o}}, G.~Mart{\'\i}nez-Mu{\~n}oz, A comparative analysis of gradient boosting algorithms, Artificial Intelligence Review 54 (2021) 1937--1967.

\bibitem{alshourbaji2023efficient}
I.~AlShourbaji, N.~Helian, Y.~Sun, A.~G. Hussien, L.~Abualigah, B.~Elnaim, An efficient churn prediction model using gradient boosting machine and metaheuristic optimization, Scientific Reports 13~(1) (2023) 14441.

\bibitem{paliwal2022xgbrs}
S.~Paliwal, A.~K. Mishra, R.~K. Mishra, N.~Nawaz, M.~Senthilkumar, Xgbrs framework integrated with word2vec sentiment analysis for augmented drug recommendation., Computers, Materials \& Continua 72~(3) (2022).

\bibitem{sina2022model}
S.~M. Sina~Mirabdolbaghi, B.~Amiri, Model optimization analysis of customer churn prediction using machine learning algorithms with focus on feature reductions, Discrete Dynamics in Nature and Society 2022~(1) (2022) 5134356.

\bibitem{asif2025data}
D.~Asif, M.~S. Arif, A.~Mukheimer, A data-driven approach with explainable artificial intelligence for customer churn prediction in the telecommunications industry, Results in Engineering 26 (2025) 104629.

\bibitem{amekoe2024exploring}
K.~M. Amekoe, H.~Azzag, Z.~C. Dagdia, M.~Lebbah, G.~Jaffre, Exploring accuracy and interpretability trade-off in tabular learning with novel attention-based models, Neural Computing and Applications 36~(30) (2024) 18583--18611.

\bibitem{ren2019deep}
K.~Ren, J.~Qin, L.~Zheng, Z.~Yang, W.~Zhang, L.~Qiu, Y.~Yu, Deep recurrent survival analysis, in: Proceedings of the AAAI conference on artificial intelligence, Vol.~33, 2019, pp. 4798--4805.

\end{thebibliography}
